Automated Model Discovery via Multi-modal & Multi-step Pipeline

Automated model discovery is the process of automatically searching and identifying the most appropriate model for a given dataset over a large combinatorial search space. Existing approaches, however, often face challenges in balancing the capture of fine-grained details with ensuring generalizability beyond training data regimes with a reasonable model complexity. In this paper, we present a multi-modal \& multi-step pipeline for effective automated model discovery. Our approach leverages two vision-language-based modules (VLM), AnalyzerVLM and EvaluatorVLM, for effective model proposal and evaluation in an agentic way. AnalyzerVLM autonomously plans and executes multi-step analyses to propose effective candidate models. EvaluatorVLM assesses the candidate models both quantitatively and perceptually, regarding the fitness for local details and the generalibility for overall trends. Our results demonstrate that our pipeline effectively discovers models that capture fine details and ensure strong generalizability. Additionally, extensive ablation studies show that both multi-modality and multi-step reasoning play crucial roles in discovering favorable models.

==> Tables/ablation.tex <==
% \begin{table*}[ht!]
% \renewcommand{\arraystretch}{0.8}
%   \caption{\textbf{Ablation study on the each module: VLM score, VLM analyzer, and the island adoption.} Comparison of our model with each modules. Starting from the greedy search of automatic statistician, as the pool-based search is utilized, the performance increases. With the help of VLM on model evaluation and model suggestion, the performance increases more. With the islands, it shows the best result at most datasets.}
%   \centering
%   \resizebox{0.9\linewidth}{!}{\begin{tabular}{lccccc}
%     \toprule
%     Dataset & AutoStats. & +Pool search & +VLM score & +VLM analyzer & +Island\\
%     \cmidrule{1-6}

%     Airline& 0.235 & 0.075 & 0.075 & \textbf{0.055} & \textbf{0.055}   \\
%     Solar irradiance & 0.200 & 0.157 & 0.086 & \textbf{0.057} & 0.174 \\
%     Mauna Loa & 0.020 & 0.032 & 0.034 & \textbf{0.007} & \textbf{0.007}  \\
%     Wheat  & 0.134 & 0.134 & 0.161 & 0.015 & \textbf{0.013}  \\
%     Internet & 0.164 & 0.055 & 0.048 & \textbf{0.036} & 0.048  \\
    
%     % \midrule
%     % Random Choice & 50.0 & 50.0 & 50.0 & 50.0 & 50.0 & 50.0 & 50.0 & 50.0 & 50.0 & 50.0 \\
%     \bottomrule
%   \end{tabular}}
%   \label{tab:ablation}
%   \vspace{-2mm}
% \end{table*}

% \begin{table}[H]
\begin{table*}[ht!]
\renewcommand{\arraystretch}{0.8}
% \tiny
  \caption{\textbf{Ablation study on the each module: VLM score, VLM analyzer, and the island adoption.} Comparison of our model with each modules. Starting from the greedy search of automatic statistician, as the pool-based search is utilized, the performance increases. With the help of VLM on model evaluation and model suggestion, the performance increases more. With the islands, it shows the best result at most datasets.}
  \centering
  \resizebox{0.95\linewidth}{!}{\begin{tabular}{L{24mm}C{23mm}C{23mm}C{23mm}C{23mm}C{23mm}}
    \toprule
    \multirow{3}{*}{Method} & \multicolumn{5}{c}{Dataset}\\
    \cmidrule{2-6}
     & Airline & Solar Irradiance & Mauna Loa & Wheat & Internet \\
    \cmidrule{1-6}

    AutoStats. & 0.235 & 0.200 & 0.020 & 0.055 & 0.055   \\
    +Pool Search & 0.075 & 0.157 & 0.032 & 0.134 & 0.055 \\
    +VLM Score & 0.075 & 0.086 & 0.034 & 0.161 & 0.048  \\
    +VLM Analyzer & \textbf{0.055} & \textbf{0.057} & \textbf{0.007} & 0.015 & \textbf{0.036}  \\
    +Island & \textbf{0.055} & 0.174 & \textbf{0.007} & \textbf{0.013} & 0.048  \\
    
    % \midrule
    % Random Choice & 50.0 & 50.0 & 50.0 & 50.0 & 50.0 & 50.0 & 50.0 & 50.0 & 50.0 & 50.0 \\
    \bottomrule
  \end{tabular}}
  \label{tab:ablation}
  \vspace{-2mm}
\end{table*}
% \end{table}[H]

==> Tables/qualitative.tex <==
\begin{table*}[htb!]
% \begin{table}[H]
% \tiny
\renewcommand{\arraystretch}{0.8}
  \caption{\textbf{Quantitative result.} This is the extrapolation test's result at 5 univariate dataset. PER. kernel and SE. kernel is the fixed kernel, and AutoStats mean the automatic statistician. N-Beats~\cite{nbeats} is the neural time-series forecasting model. The bold number is the first ranked, and the underlined number is the second ranked. As shown in table, our method is ranked mostly at top 1 and 2, implying the effectiveness of our models.}
  \centering
  \resizebox{0.9\linewidth}{!}{\begin{tabular}{lcccc}
    \toprule
    Dataset & PER. kernel & SE. kernel & AutoStats. & Ours \\
    \cmidrule{1-5}

    Airline & \textbf{0.019} & 0.495 & 0.075  & \underline{0.055}   \\
    Solar irradiance & 0.490 & 0.442 & \textbf{0.157}  & \underline{0.174} \\
    Mauna Loa & \textbf{0.006} & \textbf{0.006} & 0.034 & \underline{0.007}  \\
    Wheat & \underline{0.068} & 0.294 & 0.134 &  \textbf{0.013}  \\
    Internet & 0.137 & 0.136 & \underline{0.055} & \textbf{0.049}  \\
    
    % \midrule
    % Random Choice & 50.0 & 50.0 & 50.0 & 50.0 & 50.0 & 50.0 & 50.0 & 50.0 & 50.0 & 50.0 \\
    \bottomrule
  \end{tabular}}
  \label{tab:quantitative}
  \vspace{-2mm}
\end{table*}
% \end{table}

% \begin{table*}[!hbt]
% % \begin{table}[H]
% % \tiny
% \renewcommand{\arraystretch}{0.8}
%   \caption{\textbf{Quantitative result.} This is the extrapolation test's result at 5 univariate dataset. PER. kernel and SE. kernel is the fixed kernel, and AutoStats mean the automatic statistician. The bold number is the first ranked, and the underlined number is the second ranked. As shown in table, our method is ranked mostly at top 1 and 2, implying the effectiveness of our models.}
%   \centering
%   \resizebox{0.95\linewidth}{!}{\begin{tabular}{L{20mm}C{23mm}C{23mm}C{23mm}C{23mm}C{23mm}}
%     \toprule
%     \multirow{3}{*}{Method} & \multicolumn{5}{c}{Dataset}\\
%     \cmidrule{2-6}
%      & Airline & Solar Irradiance & Mauna Loa & Wheat & Internet \\
%     \midrule

%     PER. kernel & \textbf{0.019} & 0.490 & \textbf{0.006} & \underline{0.068} & 0.137   \\
%     SE. kernel & 0.495 & 0.442 & \textbf{0.006} & 0.294 & 0.136 \\
%     AutoStats. & 0.235 & \underline{0.200} & 0.020 &0.134 & \underline{0.055}  \\
%     Ours & \underline{0.055} & \textbf{0.174} & \underline{0.007} & \textbf{0.013} & \textbf{0.049}  \\
    
%     % \midrule
%     % Random Choice & 50.0 & 50.0 & 50.0 & 50.0 & 50.0 & 50.0 & 50.0 & 50.0 & 50.0 & 50.0 \\
%     \bottomrule
%   \end{tabular}}
%   \label{tab:quantitative}
%   % \vspace{-2mm}
% \end{table*}
% % \end{table}

==> Tables/vision-score-prompt.tex <==

% \begin{table*}[ht!]
% \renewcommand{\arraystretch}{0.8}
%   \caption{\textbf{Prompt} }
%   \centering
%   \resizebox{0.9\linewidth}{!}{\begin{tabular}{lc}
%     \toprule
%     % testtest & test \\
%     % 1 & 2 \\
%     You will evaluate how well the predicted kernel (red line) matches the real data (black line) by assigning a score from 0 to 100. This score will be based on two aspects: how well the red line (posterior mean value of the Gaussian process) follows the black line (real data), and how large the blue shaded area (confidence interval) is. Follow the steps below to complete the task.
%     1. Evaluate the Match Between Real Data (Black Line) and Mean Prediction (Red Line)
%     Match scores should be assigned based on how well the red line follows the black line. Please check the mean(red line) is almost overlapped to the data(black line) (then assign 40-50 points), or the mean and data samples are overlapped but shows some difference(20-40 points), not overlapped and shows only overall linear trend (10-20 points), or not following the trend at all (0-10 points). If the black line is linear and the value is 0, it is considered not following the trend at all, so assign 0 points.
%     2. Evaluate the Size of the Confidence Interval (Blue Shaded Area)
%     Confidence scores should be assigned based on the size of the blue shaded area. Please check the confidence area is small or almost hard to see across all x values (this case assign 40-50 points). shaded area is small across most x values (20-40 points), small in the middle of graph but high uncertainty at the boundaries (10-20 points), large over a significant range of y values(0-10 points). Please avoid giving the score 30 everytime, and consider the confidence interval. & \\
%     \bottomrule
%   \end{tabular}}
%   \label{tab:vision-score-prompt}
%   \vspace{-2mm}
% \end{table*}
\begin{table}[!hbt]
\centering
\caption{\textbf{Prompt for audio-visual information disentanglement.} The provided prompt is fed into GPT4 to disentangle the given content into five different audio-visual information. 
}
\begin{tabular}{p{14cm}}
\toprule
You will evaluate how well the predicted kernel (red line) matches the real data (black line) by assigning a score from 0 to 100. This score will be based on two aspects: how well the red line (posterior mean value of the Gaussian process) follows the black line (real data), and how large the blue shaded area (confidence interval) is. Follow the steps below to complete the task.\\
1. Evaluate the Match Between Real Data (Black Line) and Mean Prediction (Red Line) \\
Match scores should be assigned based on how well the red line follows the black line. Please check the mean(red line) is almost overlapped to the data(black line) (then assign 40-50 points), or the mean and data samples are overlapped but shows some difference(20-40 points), not overlapped and shows only overall linear trend (10-20 points), or not following the trend at all (0-10 points). If the black line is linear and the value is 0, it is considered not following the trend at all, so assign 0 points. \\
% 2. Evaluate the Size of the Confidence Interval (Blue Shaded Area) \\
% Confidence scores should be assigned based on the size of the blue shaded area. Please check the confidence area is small or almost hard to see across all x values (this case assign 40-50 points). shaded area is small across most x values (20-40 points), small in the middle of graph but high uncertainty at the boundaries (10-20 points), large over a significant range of y values(0-10 points). Please avoid giving the score 30 everytime, and consider the confidence interval. & \\
\bottomrule
    \end{tabular}
    \label{tab:vision-score-prompt}
\end{table}

